The complete HEFT Lagrangian after the LHC Run I

The complete effective chiral Lagrangian for a dynamical Higgs is presented and constrained by means of a global analysis including electroweak precision data together with Higgs and triple gauge boson coupling data from the LHC Run~I. The operators' basis up to next-to-leading order in the expansion consists of 148 (188 considering right-handed neutrinos) flavour universal terms and it is presented here making explicit the custodial nature of the operators. This effective Lagrangian provides the most general description of the physical Higgs couplings once the electroweak symmetry is assumed, and it allows for deviations from the $SU(2)_L$ doublet nature of the Standard Model Higgs. The comparison with the effective linear Lagrangian constructed with an exact $SU(2)_L$ doublet Higgs and considering operators with at most canonical dimension six is presented. A promising strategy to disentangle the two descriptions consists in analysing i) anomalous signals present only in the chiral Lagrangian and not expected in the linear one, that are potentially relevant for LHC searches, and ii) decorrelation effects between observables that are predicted to be correlated in the linear case and not in the chiral one. The global analysis presented here, that includes several kinematic distributions, is crucial for reducing the allowed parameter space and for controlling the correlations between parameters. This improves previous studies aimed at investigating the Higgs Nature and the origin of the electroweak symmetry breaking.

==> Fdiagrams/Ahnn.tex <==
\begin{fmffile}{Fdiagrams/ahnncoupl}
\begin{fmfgraph*}(35,25)
\fmfset{arrow_len}{2mm}
\fmfleft{i1,i2,i3,i4}
\fmfright{o4,o3,o2,o1}
  \fmf{boson}{i1,v1}
  \fmf{dashes}{i4,v1}
  \fmf{fermion}{o1,v1}
  \fmf{fermion}{v1,o4}
  
\fmfv{lab=$A^\mu$}{i1}
\fmfv{lab=$h$}{i4}
\fmfv{lab=$\nu$}{o1,o4}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/Ann.tex <==
\begin{fmffile}{Fdiagrams/anncoupl}
\begin{fmfgraph*}(35,25)
\fmfset{arrow_len}{2mm}
\fmfleft{i1,i2,i3}
\fmfright{o3,o2,o1}
  \fmf{boson}{i2,v1}
  \fmf{fermion}{o1,v1}
  \fmf{fermion}{v1,o3}
  
\fmfv{lab=$A^\nu$}{i2}
\fmfv{lab=$\nu$}{o1,o3}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/ZZZh.tex <==

\begin{fmffile}{Fdiagrams/zzzhcoupl}
\begin{fmfgraph*}(35,25)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{dashes}{i2,v1}
  \fmf{boson}{i1,v1}
  \fmf{boson}{v1,o1}
  \fmf{boson}{v1,o2}
  
\fmfv{lab=$Z_\mu$}{o1}
\fmfv{lab=$Z_\nu$}{o2}
\fmfv{lab=$Z_\rho$}{i1}
\fmfv{lab=$h$}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/ZZnn.tex <==
\begin{fmffile}{Fdiagrams/zznncoupl}
\begin{fmfgraph*}(35,25)
\fmfset{arrow_len}{2mm}
\fmfleft{i1,i2,i3,i4}
\fmfright{o4,o3,o2,o1}
  \fmf{boson}{i1,v1}
  \fmf{boson}{i4,v1}
  \fmf{fermion}{o1,v1}
  \fmf{fermion}{v1,o4}
  
\fmfv{lab=$Z^\mu$}{i1}
\fmfv{lab=$Z^\nu$}{i4}
\fmfv{lab=$\nu$}{o1,o4}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/Zhnn.tex <==
\begin{fmffile}{Fdiagrams/zhnncoupl}
\begin{fmfgraph*}(35,25)
\fmfset{arrow_len}{2mm}
\fmfleft{i1,i2,i3,i4}
\fmfright{o4,o3,o2,o1}
  \fmf{boson}{i1,v1}
  \fmf{dashes}{i4,v1}
  \fmf{fermion}{o1,v1}
  \fmf{fermion}{v1,o4}
  
\fmfv{lab=$Z^\mu$}{i1}
\fmfv{lab=$h$}{i4}
\fmfv{lab=$\nu$}{o1,o4}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/hhhh.tex <==
\begin{fmffile}{Fdiagrams/hhhhcoupl}
\begin{fmfgraph*}(35,25)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{dashes,label=$p_{h1}$}{i2,v1}
  \fmf{dashes,label=$p_{h2}$}{i1,v1}
  \fmf{dashes,label=$p_{h3}$,l.side=right}{v1,o1}
  \fmf{dashes,label=$p_{h4}$,l.side=right}{v1,o2}
  
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$h$,l.angle=0}{o2}
\fmfv{lab=$h$,l.angle=180}{i1}
\fmfv{lab=$h$,l.angle=180}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/hhnn.tex <==
\begin{fmffile}{Fdiagrams/hhnncoupl}
\begin{fmfgraph*}(35,25)
\fmfset{arrow_len}{2mm}
\fmfleft{i1,i2,i3,i4}
\fmfright{o4,o3,o2,o1}
  \fmf{dashes}{i1,v1}
  \fmf{dashes}{i4,v1}
  \fmf{fermion}{o1,v1}
  \fmf{fermion}{v1,o4}
  
\fmfv{lab=$h$}{i1,i4}
\fmfv{lab=$\nu$}{o1,o4}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/hnn.tex <==
\begin{fmffile}{Fdiagrams/hnncoupl}
\begin{fmfgraph*}(35,25)
\fmfset{arrow_len}{2mm}
\fmfleft{i1,i2,i3}
\fmfright{o3,o2,o1}
  \fmf{dashes}{i2,v1}
  \fmf{fermion}{o1,v1}
  \fmf{fermion}{v1,o3}
  
\fmfv{lab=$h$}{i2}
\fmfv{lab=$\nu$}{o1,o3}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/hqq.tex <==
\begin{fmffile}{Fdiagrams/hqqcoupl}
\begin{fmfgraph*}(30,30)
\fmfset{arrow_len}{2mm}
\fmfleft{i1,i2,i3}
\fmfright{o3,o2,o1}
  \fmf{dashes}{i2,v1}
  \fmf{fermion,label=$f_\beta$}{o1,v1}
  \fmf{fermion,label=$f_\alpha$}{v1,o3}
  
\fmfv{lab=$h$}{i2}
\end{fmfgraph*}
\end{fmffile}

